FTP: A Fine-grained Token-wise Pruner for Large Language Models via Token Routing

Recently, large language models (LLMs) have demonstrated superior performance across various tasks by adhering to scaling laws, which significantly increase model size. However, the huge computation overhead during inference hinders the deployment in industrial applications. Many works leverage traditional compression approaches to boost model inference, but these always introduce additional training costs to restore the performance and the pruning results typically show noticeable performance drops compared to the original model when aiming for a specific level of acceleration. To address these issues, we propose a fine-grained token-wise pruning approach for the LLMs, which presents a learnable router to adaptively identify the less important tokens and skip them across model blocks to reduce computational cost during inference. To construct the router efficiently, we present a search-based sparsity scheduler for pruning sparsity allocation, a trainable router combined with our proposed four low-dimensional factors as input and three proposed losses. We conduct extensive experiments across different benchmarks on different LLMs to demonstrate the superiority of our method. Our approach achieves state-of-the-art (SOTA) pruning results, surpassing other existing pruning methods. For instance, our method outperforms BlockPruner and ShortGPT by approximately 10 points on both LLaMA2-7B and Qwen1.5-7B in accuracy retention at comparable token sparsity levels.

==> backup_tables/backup_main_results_09_24.tex <==
% =======================
% MEMO.
% 1. All are `acc_norm`, including ARC series, i.e., arc-e, arc-c, please remmeber to check reported print-lines.
% 2. MMLU is a 5-shots setting
% 3. Others are 0-shot
% =======================

\begin{table}[ht]
\label{table:main}
\centering
\adjustbox{max width=0.9\textwidth}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\toprule
\tbf{Model} & \tbf{Method} & \tbf{Ratio (\%)} & \tbf{ARC-c} & \tbf{ARC-e} & \tbf{HellaSwag} & \tbf{MMLU} & \tbf{WinoGrande} & \tbf{Avg. Percentage (\%)} \\
\midrule

\multirow{9}{*}[0em]{Llama2-7B}
& \rowg Dense                 & 0     & 46.16 & 74.54 & 75.99 & 45.39 & 69.06 &  100           \\
& LaCo                  & 21.02 & 35.84 & 55.39 & 54.08 & -     & 60.46 &  77.67           \\
& RM                    & 21.02 & 22.53 & 34.43 & 29.22 & -     & 49.25 &  51.19           \\
& LLMPruner             & 27.0  & -     & -     & 60.21 & 23.33 & -     &  65.32           \\
& SliceGPT              & 21.45 & 37.12 & 63.64 & 56.04 & -     & 59.91 &  81.57           \\
& ShortGPT              & 27.0  & 32.68 & 48.61 & 56.15 & 44.51 & 64.33 &  80.22           \\
& BlockPruner           & 20.99 & 35.92 & 61.20 & 66.04 & 34.30 & 64.09 &  83.03           \\
& \tbf{FTP (static)} & 22.0    & 44.88 & 72.31 & 72.66 & 45.83 & \tbf{69.53} &  98.30           \\
& \tbf{FTP}          & 22.0    & \tbf{45.31} & \tbf{73.06} & \tbf{74.46} & \tbf{46.15} & 69.22 &  \tbf{99.21}           \\
& \tbf{FTP}          & 30.0    & 43.65 & 72.31 & 67.37 & 46.07 & 68.97 &  96.32 \\
\midrule
\multirow{8}{*}[0em]{Llama2-13B}
& \rowg Dense                 & 0     & 49.23 & 77.36 & 79.36 & 54.94 & 72.14 &  100           \\
& LaCo                  & 24.37 & 34.56 & 54.34 & 60.44 & -     & 59.27 &   74.69          \\
& RM                    & 24.37 & 41.98 & 66.12 & 66.80 & -     & 66.61 &   86.81          \\
& SliceGPT              & 21.52 & 42.41 & 68.52 & 60.71 & -     & 65.59 &   85.53          \\
& ShortGPT              & 24.60 & 42.92 & 63.55 & 69.27 & 53.83 & 69.85 &  90.28           \\
& BlockPruner           & 24.31 & 40.53 & 63.55 & 71.93 & 47.84 & 70.40 &  87.96       \\
& \tbf{FTP (static)} & 25.0    &  47.95 &  74.58     &  76.65     &  54.51     &  71.19   &   97.66         \\
& \tbf{FTP}          & 25.0    & \tbf{48.98} & \tbf{75.55} & \tbf{77.49} & \tbf{54.56} & \tbf{72.22} & \tbf{98.84}      \\
& \tbf{FTP}          & 30.0    & 48.38 & 74.75 & 75.99 & 54.47 & 71.67 &  97.83      \\
\midrule
\multirow{7}{*}[0em]{Qwen1.5-7B}
& \rowg Dense                 & 0     & 42.66 & 62.16 & 76.92 & 60.52 & 66.46 &  100           \\
& LaCo                  & 20.97 & 32.85 & 46.89 & 56.35 & -     & 58.64 &   78.48          \\
& RM                    & 20.97 & 28.58 & 54.17 & 42.00 & -     & 49.88 &   70.95          \\
& ShortGPT              & 21.88 & 33.79 & 48.44 & 63.09 & 49.54 & 60.93 &  82.54          \\
& BlockPruner           & 21.83 & 33.02 & 53.49 & 57.29 & 28.51 & 56.99 &  74.16           \\
& \tbf{FTP (static)} & 22.0  & 43.52 & 62.71 & 71.89 & 60.26 & 65.19 &  98.80     \\
& \tbf{FTP}          & 22.0    & \tbf{43.69} & \tbf{62.81} & \tbf{74.02} & \tbf{60.86} & \tbf{67.32} &  \tbf{100.03}\\
& \tbf{FTP}          & 30.0    & 40.96 & 59.60 & 68.47 & 60.77 & 65.67 &  96.03         \\
\midrule
\end{tabular}
}
\caption{\tbf{Downstream tasks performance.} FTP surpasses all the competitors under the approximate sparsity constraint. MMLU uses a 5-shot evaluation, and other tasks are all 0-shot.}
\label{tab:main_results}
\vspace{-2mm}
\end{table}



% \begin{table}[ht]
% \centering
% \adjustbox{max width=\textwidth}{
% \begin{tabular}{lcccccccccc}
% \toprule
% \tbf{Model} & \tbf{Method} & \tbf{Ratio (\%)} & \tbf{MMLU} & \tbf{PIQA} & \tbf{WinoGrande} & \tbf{HellaSwag} & \tbf{ARC-e} & \tbf{ARC-c} & \tbf{Avg. Score} \\
% \midrule
% \multirow{3}{*}[0em]{Llama2-7B} & Dense & 0    & 45.39 & 79.05    & 69.06 & 75.99 & 74.54 & 46.16 & 68.96 \\
%                                   & FTP   & 29.9 & 45.69 & $\times$ & 68.59 & $\times$ & 72.31 & 42.21 & $\times$ \\
%                                   & FTP   & 39.9 & 45.56 & $\times$ & 68.59 & $\times$ & 72.31 & 42.21 & $\times$ \\
% \midrule
% \multirow{3}{*}[0em]{Llama3-8B} & Dense & 0    & 65.28  & 80.79    & 72.85 & 79.19 & 77.69 & 53.33 & $\times$ \\
%                                   & FTP   & 29.9 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
%                                   & FTP   & 39.9 & 63.72  & 64.15    & 69.30 & 54.89 & 67.17 & 43.00 & $\times$ \\
% \midrule
% \multirow{2}{*}[0em]{Qwen1.5-7B} & Dense & 0    & 60.52 & $\times$ & 66.06 & $\times$ & 62.29 & 42.83 & $\times$ \\
%                                    & FTP   & 29.9 & 60.79 & $\times$ & 63.93 & $\times$ & 58.63 & 40.53 & $\times$ \\
% \bottomrule
% \end{tabular}
% }
% \caption{Performance comparison of different models and pruning methods across multiple benchmarks.}
% \label{tab:performance_comparison}
% \end{table}

% llama2-7B
% & RM          & 20.97 & -     & 67.36 & 49.88 & 42.00 & 54.17 & 28.58 &            \\
% & ATP         & 30    & 38.32 & -     & -     & -     & -     & -     &            \\

==> backup_tables/efficiency.tex <==
\begin{table}[ht]
\scriptsize
\centering
\adjustbox{max width=0.65\textwidth}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Method} &\textbf{Ratio(\%)} & \textbf{Generated Tokens} & \textbf{KV Cache} &\textbf{Infer time (\%)} \\
\midrule
Dense                & 0   & 1000  & False & 100\% \\
FTP                  & 30  & 1000  & False & 127.91\% \\
FTP                  & 40  & 1000  & False & 140.76\% \\
\midrule
Dense                & 0   & 2000  & False & 100\% \\
FTP                  & 30  & 2000  & False & 138.68\% \\
FTP                  & 40  & 2000  & False & 160.63\% \\
\bottomrule
\end{tabular}
}
\caption{Comparison of actual speedup of inference time in Llama2-7B.}
\label{tab:efficiency}
\end{table}

==> backup_tables/features.tex <==
\begin{table}[ht]
\label{table:feature}
\centering
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Method}  & \textbf{MMLU} &  \textbf{ARC-c} & \textbf{Percentage} \\
\midrule
\midrule
Dense          & 45.39 & 46.16 & 100 \\
HF w.o. position     & 44.59 & 30.72 & 82.26\\
HF w.o. attn      & 45.43 & 41.21 & 94.64\\
HF w.o. sparsity      & 45.79 & 38.51 & 92.08 \\
Hidden states      & 44.78 & 33.87  & 85.91\\
HF w. Hidden states     & 44.99 & 34.57 & 86.90\\
HF   & \textbf{45.69} &  \textbf{42.21} & 96.01\\
\bottomrule
\end{tabular}
}
\caption{Comparisons of different inputs.}
\label{tab:comparison}
\end{table}

==> backup_tables/old_main_results.tex <==
{'layer_9': 0.896, 'layer_10': 0.8909, 'layer_11': 0.8392, 'layer_12': 0.8416, 'layer_13': 0.8363, 'layer_14': 0.752, 'layer_15': 0.7329, 'layer_16': 0.693, 'layer_17': 0.6239, 'layer_18': 0.6011, 'layer_19': 0.4913, 'layer_20': 0.4694, 'layer_21': 0.3628, 'layer_22': 0.303, 'layer_23': 0.2948, 'layer_24': 0.3001, 'layer_25': 0.3031, 'layer_26': 0.313, 'layer_27': 0.301, 'layer_28': 0.2778, 'layer_29': 0.2853, 'layer_30': 0.292, 'layer_31': 0.2991, 'layer_32': 0.2994, 'layer_33': 0.2503, 'layer_34': 0.2531, 'layer_35': 0.2522, 'layer_36': 0.242, 'layer_37': 0.2394, 'layer_38': 0.429}

==> backup_tables/old_old_main_results.tex <==
% =======================
% MEMO.
% 1. All are `acc_norm`, including ARC series, i.e., arc-e, arc-c, please remmeber to check reported print-lines.
% 2. MMLU is a 5-shots setting
% 3. Others are 0-shot
% =======================
% TODO:
% 1. 列数据交换 2. 更多benchmark
\begin{table}[ht]
\label{table:main}
\centering
\adjustbox{max width=0.9\textwidth}{
\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Ratio (\%)} & \textbf{ARC-c} & \textbf{ARC-e} & \textbf{HellaSwag} & \textbf{MMLU} & \textbf{OBQA} & \textbf{WinoGrande} & \textbf{Avg. Percentage} \\
\midrule
\midrule
\multirow{9}{*}[0em]{Llama2-7B}
& Dense                 & 0     & 46.16 & 74.54 & 75.99 & 45.39 &      & 69.06 &             \\
& LaCo                  & 21.02 & 35.84 & 55.39 & 54.08 & -     & -    & 60.46 &             \\
& RM                    & 21.02 & 22.53 & 34.43 & 29.22 & -     & -    & 49.25 &             \\
& LLMPruner             & 27.0  & -     & -     & 60.21 & 23.33 & -    & -     &             \\
& SliceGPT              & 21.45 & 37.12 & 63.64 & 56.04 & -     & -    & 59.91 &             \\
& ShortGPT              & 27.0  & 32.68 & 48.61 & 56.15 & 44.51 &      & 64.33 &             \\
& BlockPruner           & 20.99 & 35.92 & 61.20 & 66.04 & 34.30 &      & 64.09 &             \\
& \textbf{FTP (static)} & 22    & 44.88 & 72.31 & 72.66 & 45.83 & 42.00& 69.53 &             \\
& \textbf{FTP}          & 22    & 45.31 & 73.06 & 74.46 & 46.15 & 41.40& 69.22 &             \\
& \textbf{FTP}          & 30    & 42.21 & 72.31 & 67.37 & 45.69 &      & 68.03 &             \\
\midrule
\multirow{8}{*}[0em]{Llama2-13B}
& Dense                 & 0     & 49.23 & 77.36 & 79.36 & 54.94 &      & 72.14 &             \\
& LaCo                  & 24.37 & 34.56 & 54.34 & 60.44 & -     & -    & 59.27 &             \\
& RM                    & 24.37 & 41.98 & 66.12 & 66.80 & -     & -    & 66.61 &             \\
& SliceGPT              & 21.52 & 42.41 & 68.52 & 60.71 & -     & -    & 65.59 &             \\
& ShortGPT              & 24.60 & 42.92 & 63.55 & 69.27 & 53.83 &      & 69.85 &             \\
& BlockPruner           & 24.31 & 40.53 & 63.55 & 71.93 & 47.84 &      & 70.40 &             \\
& \textbf{FTP (static)} & 25    &       &       &       &       &      &       &             \\
& \textbf{FTP}          & 25    & 48.98 & 75.93 & 77.66 & 54.50 &      & 71.11 &             \\
& \textbf{FTP}          & 30    & 48.38 & 74.75 & 75.99 & 54.47 &      & 71.67 &             \\
\midrule
\multirow{7}{*}[0em]{Qwen1.5-7B}
& Dense                 & 0     & 42.66 & 62.16 & 76.92 & 60.52 & 41.6 & 66.46 &             \\
& LaCo                  & 20.97 & 32.85 & 46.89 & 56.35 & -     & -    & 58.64 &             \\
& RM                    & 20.97 & 28.58 & 54.17 & 42.00 & -     & -    & 49.88 &             \\
& ShortGPT              & 21.88 & 33.79 & 48.44 & 63.09 & 49.54 &      & 60.93 &             \\
& BlockPruner           & 21.83 & 33.02 & 53.49 & 57.29 & 28.51 &      & 56.99 &             \\
& \textbf{FTP (static)} & 22    &       &       &       &       &      &       &             \\
& \textbf{FTP}          & 22    & 40.78 & 60.86 & 74.02 & 60.30 &      & 65.82 &             \\
& \textbf{FTP}          & 30    & 40.96 & 59.60 & 68.47 & 60.77 & 38.2 & 65.67 &             \\
\midrule
\end{tabular}
}
\caption{Performance comparison of different models and pruning methods across multiple benchmarks.}
\label{tab:performance_comparison}
\end{table}


==> backup_tables/router.tex <==
\begin{table}[ht]
\label{table:router}
\centering
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Method}  & \textbf{MMLU} &  \textbf{ARC-c}  & \textbf{Percentage}\\
\midrule
\midrule
Dense          & 45.39 &  46.16 & 100  \\
Recurrent router     & 45.53 & 40.23 & 93.68  \\
Local router     & 43.69 & 38.21 & 89.46  \\
Global router         & \textbf{45.69} & \textbf{42.21} & \textbf{96.01} \\
\bottomrule
\end{tabular}
}
\caption{Comparisons of different routers .}
\label{tab:comparison}
\end{table}

==> backup_tables/search.tex <==
\begin{table}[ht]
\centering
\adjustbox{max width=0.5\textwidth}{%
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Method}  & \textbf{MMLU} & \textbf{ARC-c} & \textbf{Percentage}\\
\midrule
\midrule
Dense          & 45.39  & 46.16 & 100\\
FTP w.o. searching     & 40.50  & 26.02  & 72.66\\
FTP w. BI initialization     & 45.29 & 34.81 & 87.49 \\
FTP w. searching       & 45.67  & 40.96  & 94.63\\
FTP w. searching and ratio tune       & \textbf{45.69}  & \textbf{42.21}  & 96.91\\
\bottomrule
\end{tabular}
}
\caption{Effect of pruning ratio search.}
\label{table:search}
\end{table}

==> backup_tables/sparsity_tune.tex <==
\begin{table}[ht]
\label{table:var_ratio}
\centering
\adjustbox{max width=\textwidth}{%
\begin{tabular}{lcccccccc}
\toprule
\textbf{Method}  & \textbf{MMLU} & \textbf{WiGr} & \textbf{HeSw} & \textbf{ARC-e} & \textbf{ARC-c} & \textbf{Avg. Score} & \textbf{Percentage}\\
\midrule
FTP w. initialization     & 45.29 & 60.38 &  & 64.44 & 34.81 &  & \\
FTP w. searching          & \textbf{45.69} & \textbf{68.59} &  & \textbf{72.31} & \textbf{42.21} &  & \\
FTP w. tuning     & 45.29 & 60.38 &  & 64.44 & 34.81 &  & \\
\bottomrule
\end{tabular}
}
\caption{Comparison of sparsity configuration settings across multiple benchmarks.}
\label{tab:steps_cmp}
\end{table}

==> backup_tables/tab_eff_tab_search.tex <==

\begin{table}[h!]
\scriptsize
\centering
\begin{minipage}{.45\linewidth}
\centering
\adjustbox{max width=\linewidth}{%
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Method} &\textbf{Ratio(\%)} & \dtb{\textbf{Generated}}{\textbf{Tokens}} & \dtb{\textbf{Infer}}{\textbf{Speedup}} \\

\midrule
Dense                & 0   & 1000  & 1.0\times \\
FTP                  & 30  & 1000  & 1.28\times \\
FTP                  & 40  & 1000  & 1.41\times \\
\midrule
Dense                & 0   & 2000  & 1.0\times\\
FTP                  & 30  & 2000  & 1.39\times \\
FTP                  & 40  & 2000  & 1.61\times \\
\bottomrule
\end{tabular}
}
\caption{Inference speedup of our FTP in Llama2-7B on different settings.}
\label{tab:efficiency}
\end{minipage}%
\hspace{0.05\linewidth}
\begin{minipage}{.45\linewidth}
\centering
\adjustbox{max width=\linewidth}{%
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Method}  & \textbf{ARC-c}  & \textbf{MMLU} & \textbf{Percentage}\\
\midrule

Uniform distribution      & 26.02 & 40.50   & 72.66\\
BI score based    & 34.81    & 45.29 & 87.49 \\
SRO wo finetune       & 40.96   & 45.67  & 94.63\\
SRO       & \textbf{43.65}    & \textbf{46.07}  & \textbf{98.00}\\
\bottomrule
\end{tabular}
}
\caption{Ablations of sparsity ratio optimization strategy. Under 30\% sparsity, comparisons on Llama2-7B.}
\label{tab:search}
\end{minipage}
\end{table}




==> backup_tables/tab_router_and_tab_features.tex <==
\begin{table}[h!]
\scriptsize
\centering
\begin{minipage}{.45\linewidth}
\centering
\adjustbox{max width=\linewidth}{%
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Method} &  \textbf{ARC-c} & \textbf{MMLU} & \textbf{Percentage} \\
\midrule

Dense & 46.16  & 45.39  & 100 \\
Hidden states & 33.87  & 44.78 & 85.91 \\
HF w. hidden states & 34.57  & 44.99 & 86.90 \\
HF w.o. position  & 30.72 & 44.59 & 82.26 \\
HF w.o. attntion score  & 41.21 & 45.43 & 94.64 \\
HF w.o. attntion rank  & 42.37 &  &  \\
HF w.o. sparsity  & 38.51 & 45.79 & 92.08 \\

HF  & 43.65  & 46.07 & 98.00 \\
\bottomrule
\end{tabular}}
\caption{Overall comparisons of different inputs, HF indicates our proposed hybrid feature.}
\label{tab:feature}
\end{minipage}%
\hspace{0.05\linewidth}
\begin{minipage}{.45\linewidth}
\centering
\adjustbox{max width=\linewidth}{%
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Method}  & \textbf{ARC-c} & \textbf{MMLU} & \textbf{Percentage} \\
\midrule

Recurrent router  & 40.23  & 45.53 & 93.68 \\
Local router  & 38.21 & 43.69 & 89.46 \\
Global router  & \textbf{ 43.65} & \textbf{46.07} & \textbf{98.00} \\
\bottomrule
\end{tabular}}
\caption{Overall comparisons of different routers.}
\label{tab:router}
\end{minipage}
\end{table}

==> backup_tables/various_sparsity.tex <==
\begin{table}[ht]
\centering
\adjustbox{max width=0.85\textwidth}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Ratio (\%)} & \textbf{ARC-c} & \textbf{ARC-e} & \textbf{HellaSwag} & \textbf{MMLU}& \textbf{OBQA} & \textbf{WinoGrande} & \textbf{Avg. Percentage (\%)} \\
%& SR & ARC-c & ARC-e & HellaSwag & MMLU & WinoGrande & Avg. Percentage (\%)
\midrule
\midrule
\multirow{3}{*}[0em]{Llama2-7B}
& 0  & 46.16 & 74.54 & 75.99 & 45.39 &       & 69.06 & 100               \\
& 30 & 42.21 & 72.31 & 67.37 & 45.69 &       & 68.03 & 93.52                \\
& 40 & 40.02 & 70.01 & 62.67 & 46.56 &       & 66.03 & 90.25                \\

\midrule

\multirow{3}{*}[0em]{Llama2-13B} 
& 0  & 49.23 & 77.36 & 79.36 & 54.94 &       & 72.14 & 100           \\
& 30 & 48.38 & 74.75 & 75.99 & 54.47 &       & 71.67 & 96.13         \\
& 40 & 45.22 & 70.88 & 66.50 & 54.57 & 39.60 & 70.40 & \\

\midrule
\multirow{3}{*}[0em]{Llama3-8B}
& 0  & 53.33 & 77.69 & 79.19 & 65.28 &       & 72.85 & 100                \\
& 30 & 48.63 & 73.36 & 62.41 & 64.29 &       & 69.69 & 90.45                \\
& 40 & 43.00 & 67.17 & 54.89 & 63.72 &       & 69.30 & 84.41               \\


\midrule
\multirow{3}{*}[0em]{Qwen1.5-7B}
& 0  & 42.66 & 62.16 & 76.92 & 60.52 & 41.60 & 66.46 & 100          \\
& 30 & 40.96 & 59.60 & 68.47 & 60.77 & 38.20 & 65.67 & 94.03          \\
& 40 & 36.15 & 53.03 & 62.59 & 60.83 & 33.60 & 59.04 & 87.20\\

\bottomrule
\end{tabular}
}
\caption{Performance comparison of different models and pruning methods across multiple benchmarks.}
\label{tab:various_sparsity}
\end{table}


% 2-7b
%& 50 & 32.33 & 58.99 & 51.45 & 45.70 & 59.04 &  79.18               \\

% 3-8b
%& 50 & 38.14 & 58.75 & 47.37 &       & 57.70 &  76.18               \\



==> backup_tables/various_sparsity_2.tex <==
\begin{table}[ht]
\centering
\adjustbox{max width=0.85\textwidth}{
\begin{tabular}{l|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Ratio (\%)} & \textbf{ARC-c} & \textbf{ARC-e} & \textbf{HellaSwag} & \textbf{MMLU} & \textbf{WinoGrande} & \textbf{Avg. Percentage (\%)} \\
%& SR & ARC-c & ARC-e & HellaSwag & MMLU & WinoGrande & Avg. Percentage (\%)
\midrule

\multirow{3}{*}[0em]{Llama2-7B}
& \rowg 0  & 46.16 & 74.54 & 75.99 & 45.39 & 69.06 & 100               \\
& 30 & 43.65 & 72.31 & 67.37 & 46.07 & 68.97 & 95.90                \\
& 40 & 40.02 & 70.01 & 62.67 & 46.56 & 66.03 & 91.69                \\

\midrule

\multirow{3}{*}[0em]{Llama2-13B} 
& \rowg 0  & 49.23 & 77.36 & 79.36 & 54.94 & 72.14 & 100           \\
& 30 & 48.38 & 74.75 & 75.99 & 54.47 & 71.67 & 97.67         \\
& 40 & 45.22 & 70.88 & 66.50 & 54.57 & 70.40 & 92.36 \\

\midrule
\multirow{3}{*}[0em]{Llama3-8B}
& \rowg 0  & 53.33 & 77.69 & 79.19 & 65.28 & 72.85 & 100                \\
& 30 & 48.63 & 73.36 & 62.41 & 64.29 & 69.69 & 91.40                \\
& 40 & 43.00 & 67.17 & 54.89 & 63.72 & 69.30 & 85.57               \\


\midrule
\multirow{3}{*}[0em]{Qwen1.5-7B}
& \rowg 0  & 42.66 & 62.16 & 76.92 & 60.52 & 66.46 & 100     \\
& 30 & 40.96 & 59.60 & 68.47 & 60.77 & 65.67 & 95.71   \\
& 40 & 36.15 & 53.03 & 62.59 & 60.83 & 59.04 & 87.98   \\

\bottomrule
\end{tabular}
}
\caption{\textbf{Various sparsity ratios.} FTP still maintains relatively objective performance at higher sparsity ratio (40\%), and is even better than BlockPruner, ShortGPT and other methods on Llama2-7B with a sparsity ratio
 of 22\% (in Table \ref{tab:main_results}).}
\label{tab:var_spars}
\end{table}


% 2-7b
%& 50 & 32.33 & 58.99 & 51.45 & 45.70 & 59.04 &  79.18               \\

% 3-8b
%& 50 & 38.14 & 58.75 & 47.37 &       & 57.70 &  76.18               \\



==> tables/main_results.tex <==
% =======================
% MEMO.
% 1. All are `acc_norm`, including ARC series, i.e., arc-e, arc-c, please remmeber to check reported print-lines.
% 2. MMLU is a 5-shots setting
% 3. Others are 0-shot
% =======================

\begin{table}[ht]
\label{table:main}
\centering
\adjustbox{max width=0.9\textwidth}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\toprule
\tbf{Model} & \tbf{Method} & \tbf{Ratio (\%)} & \tbf{ARC-c} & \tbf{ARC-e} & \tbf{HellaSwag} & \tbf{MMLU} & \tbf{WinoGrande} & \tbf{Avg. Percentage (\%)} \\
\midrule

\multirow{9}{*}[0em]{Llama2-7B}
& \rowg Dense                 & 0     & 46.16 & 74.54 & 75.99 & 45.39 & 69.06 &  100           \\
& LaCo                  & 21.02 & 35.84 & 55.39 & 54.08 & -     & 60.46 &  77.67           \\
& RM                    & 21.02 & 22.53 & 34.43 & 29.22 & -     & 49.25 &  51.19           \\
& LLMPruner             & 27.0  & -     & -     & 60.21 & 23.33 & -     &  65.32           \\
& SliceGPT              & 21.45 & 37.12 & 63.64 & 56.04 & -     & 59.91 &  81.57           \\
& ShortGPT              & 27.0  & 32.68 & 48.61 & 56.15 & 44.51 & 64.33 &  80.22           \\
& BlockPruner           & 20.99 & 35.92 & 61.20 & 66.04 & 34.30 & 64.09 &  83.03           \\
& \tbf{FTP (static)} & 22.0    & 44.88 & 72.31 & 72.66 & 45.83 & \tbf{69.53} &  98.30           \\
& \tbf{FTP}          & 22.0    & \tbf{45.31} & \tbf{73.06} & \tbf{74.46} & \tbf{46.15} & 69.22 &  \tbf{99.21}           \\
& \tbf{FTP}          & 30.0    & 43.65 & 72.31 & 67.37 & 46.07 & 68.97 &  96.32 \\
\midrule
\multirow{8}{*}[0em]{Llama2-13B}
& \rowg Dense                 & 0     & 49.23 & 77.36 & 79.36 & 54.94 & 72.14 &  100           \\
& LaCo                  & 24.37 & 34.56 & 54.34 & 60.44 & -     & 59.27 &   74.69          \\
& RM                    & 24.37 & 41.98 & 66.12 & 66.80 & -     & 66.61 &   86.81          \\
& SliceGPT              & 21.52 & 42.41 & 68.52 & 60.71 & -     & 65.59 &   85.53          \\
& ShortGPT              & 24.60 & 42.92 & 63.55 & 69.27 & 53.83 & 69.85 &  90.28           \\
& BlockPruner           & 24.31 & 40.53 & 63.55 & 71.93 & 47.84 & 70.40 &  87.96       \\
& \tbf{FTP (static)} & 25.0    &  47.95 &  74.58     &  76.65     &  54.51     &  71.19   &   97.66         \\
& \tbf{FTP}          & 25.0    & \tbf{48.98} & \tbf{75.55} & \tbf{77.49} & \tbf{54.56} & \tbf{72.22} & \tbf{98.84}      \\
& \tbf{FTP}          & 30.0    & 48.38 & 74.75 & 75.99 & 54.47 & 71.67 &  97.83      \\
\midrule
\multirow{7}{*}[0em]{Qwen1.5-7B}
& \rowg Dense                 & 0     & 42.66 & 62.16 & 76.92 & 60.52 & 66.46 &  100           \\
& LaCo                  & 20.97 & 32.85 & 46.89 & 56.35 & -     & 58.64 &   78.48          \\
& RM                    & 20.97 & 28.58 & 54.17 & 42.00 & -     & 49.88 &   70.95          \\
& ShortGPT              & 21.88 & 33.79 & 48.44 & 63.09 & 49.54 & 60.93 &  82.54          \\
& BlockPruner           & 21.83 & 33.02 & 53.49 & 57.29 & 28.51 & 56.99 &  74.16           \\
& \tbf{FTP (static)} & 22.0  & 43.52 & 62.71 & 71.89 & 60.26 & 65.19 &  98.80     \\
& \tbf{FTP}          & 22.0    & \tbf{43.69} & \tbf{62.81} & \tbf{74.02} & \tbf{60.86} & \tbf{67.32} &  \tbf{100.03}\\
& \tbf{FTP}          & 30.0    & 40.96 & 59.60 & 68.47 & 60.77 & 65.67 &  96.03         \\
\midrule
\end{tabular}
}
\caption{\tbf{Downstream tasks performance.} FTP surpasses all the competitors under the approximate sparsity constraint. MMLU uses a 5-shot evaluation, and other tasks are all 0-shot.}
\label{tab:main_results}
\vspace{-2mm}
\end{table}



% \begin{table}[ht]
% \centering
% \adjustbox{max width=\textwidth}{
% \begin{tabular}{lcccccccccc}
% \toprule
% \tbf{Model} & \tbf{Method} & \tbf{Ratio (\%)} & \tbf{MMLU} & \tbf{PIQA} & \tbf{WinoGrande} & \tbf{HellaSwag} & \tbf{ARC-e} & \tbf{ARC-c} & \tbf{Avg. Score} \\
% \midrule
% \multirow{3}{*}[0em]{Llama2-7B} & Dense & 0    & 45.39 & 79.05    & 69.06 & 75.99 & 74.54 & 46.16 & 68.96 \\
%                                   & FTP   & 29.9 & 45.69 & $\times$ & 68.59 & $\times$ & 72.31 & 42.21 & $\times$ \\
%                                   & FTP   & 39.9 & 45.56 & $\times$ & 68.59 & $\times$ & 72.31 & 42.21 & $\times$ \\
% \midrule
% \multirow{3}{*}[0em]{Llama3-8B} & Dense & 0    & 65.28  & 80.79    & 72.85 & 79.19 & 77.69 & 53.33 & $\times$ \\
%                                   & FTP   & 29.9 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
%                                   & FTP   & 39.9 & 63.72  & 64.15    & 69.30 & 54.89 & 67.17 & 43.00 & $\times$ \\
% \midrule
% \multirow{2}{*}[0em]{Qwen1.5-7B} & Dense & 0    & 60.52 & $\times$ & 66.06 & $\times$ & 62.29 & 42.83 & $\times$ \\
%                                    & FTP   & 29.9 & 60.79 & $\times$ & 63.93 & $\times$ & 58.63 & 40.53 & $\times$ \\
% \bottomrule
% \end{tabular}
% }
% \caption{Performance comparison of different models and pruning methods across multiple benchmarks.}
% \label{tab:performance_comparison}
% \end{table}

% llama2-7B
% & RM          & 20.97 & -     & 67.36 & 49.88 & 42.00 & 54.17 & 28.58 &            \\
% & ATP         & 30    & 38.32 & -     & -     & -     & -     & -     &            \\

==> tables/new_main.tex <==

\begin{table}[ht]
\label{table:main}
\centering
\vspace{-4mm}
\caption{\tbf{Downstream tasks performance.} FTP surpasses all the competitors under the comparable sparsity constraint. MMLU uses a 5-shot evaluation, and other tasks are all 0-shot.}
\vspace{4mm}
\adjustbox{max width=0.9\textwidth}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\toprule
\tbf{Model} & \tbf{Method} & \tbf{Ratio (\%)} & \tbf{ARC-c} & \tbf{ARC-e} & \tbf{HellaSwag} & \tbf{MMLU} & \tbf{WinoGrande} & \tbf{Avg. Percentage (\%)} \\
\midrule

\multirow{10}{*}[0em]{LLaMA2-7B}
& \rowg Dense           & 0     & 46.16 & 74.54 & 75.99 & 45.39 & 69.06 &  100           \\
& LaCo                  & 21.02 & 35.84 & 55.39 & 54.08 & -     & 60.46 &  77.67           \\
& RM                    & 21.02 & 22.53 & 34.43 & 29.22 & -     & 49.25 &  51.19           \\
& LLMPruner             & 27.0  & -     & -     & 60.21 & 23.33 & -     &  65.32           \\
& SliceGPT              & 21.45 & 37.12 & 63.64 & 56.04 & -     & 59.91 &  81.57           \\
& LayerSkip              & 21.88 & 33.26 & 72.54 & 55.92 & 43.32 & 69.37 & 87.77            \\
& ShortGPT              & 27.0  & 32.68 & 48.61 & 56.15 & 44.51 & 64.33 &  80.22           \\
& BlockPruner           & 20.99 & 35.92 & 61.20 & 66.04 & -     & 64.09 &  84.91           \\
& \tbf{FTP (static)} & 22.0    & 44.88 & 72.31 & 72.66 & 45.83 & \tbf{69.53} &  98.30           \\
& \tbf{FTP}          & 22.0    & \tbf{45.31} & \tbf{73.06} & \tbf{74.46} & \tbf{46.15} & 69.22 &  \tbf{99.21}           \\
& \tbf{FTP}          & 30.0    & 43.65 & 72.31 & 67.37 & 46.07 & 68.97 &  96.32 \\
\midrule
\multirow{8}{*}[0em]{LLaMA2-13B}
& \rowg Dense           & 0     & 49.23 & 77.36 & 79.36 & 54.94 & 72.14 &  100           \\
& LaCo                  & 24.37 & 34.56 & 54.34 & 60.44 & -     & 59.27 &   74.69          \\
& RM                    & 24.37 & 41.98 & 66.12 & 66.80 & -     & 66.61 &   86.81          \\
& SliceGPT              & 21.52 & 42.41 & 68.52 & 60.71 & -     & 65.59 &   85.53          \\
& LayerSkip              & 22.50 & 47.85 & 77.81 & 57.88 & 52.49 & 72.06 &  93.23           \\
& ShortGPT              & 24.60 & 42.92 & 63.55 & 69.27 & 53.83 & 69.85 &  90.28           \\
& BlockPruner           & 24.31 & 40.53 & 63.55 & 71.93 & -     & 70.40 &  88.18       \\
& \tbf{FTP (static)} & 25.0    &  47.95 &  74.58     &  76.65     &  54.51     &  71.19   &   97.66         \\
& \tbf{FTP}          & 25.0    & \tbf{48.98} & \tbf{75.55} & \tbf{77.49} & \tbf{54.56} & \tbf{72.22} & \tbf{98.84}      \\
& \tbf{FTP}          & 30.0    & 48.38 & 74.75 & 75.99 & 54.47 & 71.67 &  97.83      \\
\midrule
\multirow{7}{*}[0em]{Qwen1.5-7B}
& \rowg Dense           & 0     & 42.66 & 62.16 & 76.92 & 60.52 & 66.46 &  100           \\
& LaCo                  & 20.97 & 32.85 & 46.89 & 56.35 & -     & 58.64 &   78.48          \\
& RM                    & 20.97 & 28.58 & 54.17 & 42.00 & -     & 49.88 &   70.95          \\
& ShortGPT              & 21.88 & 33.79 & 48.44 & 63.09 & 49.54 & 60.93 &  82.54          \\
& BlockPruner           & 21.83 & 33.02 & 53.49 & 57.29 & -  & 56.99 &  80.92           \\
& \tbf{FTP (static)} & 22.0  & 43.52 & 62.71 & 71.89 & 60.26 & 65.19 &  98.80     \\
& \tbf{FTP}          & 22.0    & \tbf{43.69} & \tbf{62.81} & \tbf{74.02} & \tbf{60.86} & \tbf{67.32} &  \tbf{100.03}\\
& \tbf{FTP}          & 30.0    & 40.96 & 59.60 & 68.47 & 60.77 & 65.67 &  96.03         \\
\midrule
\end{tabular}
}

\label{tab:main_results}
\vspace{-4mm}
\end{table}




